Reconstructing weighted voting schemes from partial information about their power indices

A number of recent works [Goldberg 2006; O'Donnell and Servedio 2011; De, Diakonikolas, and Servedio 2017; De, Diakonikolas, Feldman, and Servedio 2014] have considered the problem of approximately reconstructing an unknown weighted voting scheme given information about various sorts of ``power indices'' that characterize the level of control that individual voters have over the final outcome. In the language of theoretical computer science, this is the problem of approximating an unknown linear threshold function (LTF) over $\{-1, 1\}^n$ given some numerical measure (such as the function's $n$ ``Chow parameters,'' a.k.a. its degree-1 Fourier coefficients, or the vector of its $n$ Shapley indices) of how much each of the $n$ individual input variables affects the outcome of the function. In this paper we consider the problem of reconstructing an LTF given only partial information about its Chow parameters or Shapley indices; i.e. we are given only the Chow parameters or the Shapley indices corresponding to a subset $S \subseteq [n]$ of the $n$ input variables. A natural goal in this partial information setting is to find an LTF whose Chow parameters or Shapley indices corresponding to indices in $S$ accurately match the given Chow parameters or Shapley indices of the unknown LTF. We refer to this as the Partial Inverse Power Index Problem. Our main results are a polynomial time algorithm for the ($\varepsilon$-approximate) Chow Parameters Partial Inverse Power Index Problem and a quasi-polynomial time algorithm for the ($\varepsilon$-approximate) Shapley Indices Partial Inverse Power Index Problem.

==> ap-symbols.tex <==
\section{Quantities associated with an LTF}

The following table summarizes the notation that we use for a number of quantities associated with a linear threshold function $f : \pmo^n \to \pmo$ and index $i \in [n]$.

%
{\begin{center}
%
\def\arraystretch{1.5}
\begin{tabular}{l|l|l}
\textbf{Notation} & \textbf{Definition} & \textbf{Description}\\ \hline
$\fh(i)$ & $\Ex_{\bx \sim \pmo^n}[f(\bx) \cdot \bx_i]$ & The $i$th Fourier coefficient/Chow parameter of $f$. \\
$\fh(i, p)$ & $\Ex_{\bx \sim u_p^n}[f(\bx) \cdot \psi_p(\bx_i)]$ & The $i$th $p$-biased Fourier coefficient of $f$. \\
$\ft(i)$ & $\Ex_{\bx \sim N(0, 1)^n}[f(\bx) \cdot \bx_i]$ & The $i$th Hermite coefficient of $f$. \\
$\fc(i)$ & $\Ex_{\bpi \sim \mathbb{S}_n}[f(x^+(\bpi, i)) - f(x(\bpi, i))]$ & The $i$th Shapley value of $f$. \\
$\fb(i)$ & $\Ex_{\bx \sim \DShap}[f(\bx) \cdot L_i(\bx)]$ & The $i$th Shapley Fourier coefficient coordinate of $f$. \\
$\fs(i)$ & $\Ex_{\bx \sim \DShap}[f(\bx) \cdot \bx_i)]$ & The $i$th Shapley coordinate correlation coefficient of $f$. \\
%
\end{tabular}
\end{center}
}
%
%
%


==> shapley-large-crit-index.tex <==
%
\subsubsection{Case 2:  The large critical index case of the Partial Shapley Parameters Problem}
\label{sec:shapley-large-ci}

\red{Recall that $\tau^\ast = \red{FILL-IN}.$}  In this section we present a quasipolynomial time algorithm for the Partial Inverse Shapley Parameters Problem in the case in which the target $\eta$-restricted LTF $f$ has ``large'' $\tau^\ast$-critical index, specifically the $\tau^\ast$-critical index is at least $\red{FILL-IN}.$ This case critically leverages ideas from~\cite{journals/geb/DeDS17}.

%


\paragraph{The idea behind the large critical index case}
\label{subsec:large-crit-shapley-intuition}
The strategy behind our algorithm will be to show that any \red{$\eta$-restricted} LTF $f : \pmo^n \to \pmo$ with $\tau^\ast$-critical index at least  $k^\ast \red{= FILL-IN}$ must be close in Shapley distance to a $k$-junta LTF. Given this structural fact, the algorithm can then simply enumerate all LTFs on $k$ variables and check whether each one is close to $f$. 

We establish the required structural fact by (1) arguing that if the critical index $k$ is sufficiently large, then the single weight $w_{k/2}$ will have larger magnitude than the $\ell_1$ weight of the entire tail $\sum_{i=k}^n \abs{w_i}$; (2) applying an anti-concentration theorem from~\cite{journals/geb/DeDS17} to conclude that in this case the tail weights will rarely affect the sign of the affine form $\ell(x) = \sum_{i=1}^n w_i x_i \red{-\theta}$ and hence that $f(x) = \sign(\ell(x))$ is close in $\ell_1$ distance to the junta $f'(x) = \sign(\ell'(x))$ where $\ell'(x) = \sum_{i=1}^{k-1} w_i x_i \red{-\theta}$; and (3) using a pair of lemmas (Lemmas~\ref{lem:fourier-upper-bounding-shapley} and~\ref{lem:ell1-upper-bounding-fourier}) to show that the closeness of two functions in $\ell_1$ distance implies closeness in (partial) Shapley distance.

We note that in this large critical index case we do not actually use the input set of Shapley values $\set{(i, \fc(i)) : i \in S}$ except to compare them with the values of a candidate LTF.
%
%


Initially, we will apply the anticoncentration theorem \ref{thm:shapley-anti-concentration} with anti-concentration radius $r = \abs{w_{k/2}}$, where $k \geq \Omega(\log n)$ is the critical index, to get that $\Prx_{\rv{x} \sim \DShap}[\abs{\ell(x)} < \abs{w_{k/2}}]$ is small. From this we will get that if we ``zero the tail weights'' in $f(x)$ to obtain a $(k-1)$-junta $f'(x)$ then the $\ell_1$ distance \red{(with respect to the Shapley distribution $\DShap$)} between $f(x)$ and $f'(x)$ is not too large. However, our overall goal is to show that the \emph{Shapley} distance between $f(x)$ and $f'(x)$ is not too large. So, we upper bound the Shapley distance between $f$ and $f'$ by their $\ell_1$ distance (via the Fourier distance) using 
the Corollary~\ref{cor:cor-ub-shapley-by-l1}. Finally, we will use the following lemma, which appears in a number of previous works (e.g.,~\cite[Fact 25]{de2014}). \red{Given a vector $w$ of non-negative weights that are sorted by magnitude, so $|w_1| \geq \cdots \geq |w_n| \geq 0$, for $i \in [n]$ let us write $\tail_i(w)$ to denote $(\sum_{j = i}^n w_j^2)^{1/2}$.} The result says that, for weight vectors $w$ with sorted weights, this quantity decreases geometrically for $i$ less than the critical index. 
\begin{lemma}
Let $w = (w_1, \ldots, w_n) \in \R^n$ be such that $\abs{w_1} \geq \cdots \geq \abs{w_n}$, and let $1 \leq a \leq b \leq c(w, \tau)$, where $c(w, \tau)$ is the $\tau$-critical index of $w$. Then $\tail_b(w) < (1 - \tau^2)^{(b - a)/2} \cdot \tail_a(w)$.
\label{lem:geom-decreasing-tail}
\end{lemma}

\begin{proof}
By definition of the critical index, $\abs{w_i} > \tau \cdot \tail_i(w)$ for $i < c(w, \tau)$. Therefore for such an $i$, $\tail_i(w)^2 = w_i^2 + \tail_{i+1}(w)^2 > \tau^2 \cdot \tail_i(w)^2 + \tail_{i+1}(w)^2$, and so $\tail_{i+1} (w)< (1 - \tau^2)^{1/2} \cdot \tail_i(w)$. The result follows by applying this last inequality repeatedly.
\end{proof}


\paragraph{The algorithm for large critical index and its analysis}

We now turn to proving the main theorem in this subsection, which gives a quasipolynomial time algorithm for the Partial Shapley Parameters Problem in the case when the critical index of $f$ is large. We follow the strategy outlined in Section~\ref{subsec:large-crit-shapley-intuition}.
The algorithm itself is simply to enumerate all LTFs on $k$ variables, then compute (good approximations of) the Shapley indices of each such candidate LTF, and finally to compare the Shapley indices of each candidate LTF with the input Shapley indices.

%
%

\begin{theorem}
Let $f(x) = \sign(\ell(x))$ be an $\eta$-restricted LTF where $\ell(x) = \sum_{i=1}^n w_i x_i \red{-\theta}$ is a linear form with \red{$w_1 \geq \cdots \geq w_n \geq 0$} and \red{$\tau^\ast$}-critical index greater than $k^\ast$ (recall Equation (\ref{eq:k-ast})), where $\eps \geq \red{THUS-AND-SUCH}.$
There is an algorithm that, on input $\set{(i, \fc(i)) : i \in S}$ for some $S \subseteq [n]$, outputs a weights-based representation of an LTF $f'$ that satisfies $\dPS{S}(f, f') \leq O(\eps)$ and runs in $\card{S} \cdot 2^{O(k^2)} \leq \red{n^{O(\log n/\eps^{12+2\zeta})}}$ time.
\label{thm:lrg-crit-index-shapley}
\end{theorem}

\begin{proof}
We have that
\[
\norm{(w_j)_{j=k}^n}_1^2 \leq n \cdot \norm{(w_j)_{j=k}^n}_2^2 \leq n \cdot (1 - \tau^2)^{k/2} \cdot \norm{(w_j)_{j=k/2}^n}_2^2 \leq n^2 \cdot (1 - \tau^2)^{k/2} \cdot w_{k/2}^2,
\]
where the second inequality is by \Cref{lem:geom-decreasing-tail}.
So, by our choice of $k \geq 4 \log n \cdot (\log(\frac{1}{1-\tau^2}))^{-1}$,
\begin{equation}
\norm{(w_j)_{j=k}^n}_1 \leq |w_{k/2}| \ .
\label{eq:wk2-vs-w1wt}
\end{equation}

Define $\ell'(x) =\sum_{i=1}^{k-1} w_i x_i \red{-\theta}$ and $f'(x) = \sign(\ell'(x))$. We can assume without loss of generality that $|\ell(x)| \neq |\ell(x) - \ell'(x)|$ \red{for all $x \in \bn$}. If not, we can ensure this by perturbing the threshold in one of $\ell(x)$, $\ell'(x)$ slightly without changing the values of $f(x)$, $f'(x)$ for any $x$.
Then
\begin{align*}
\Prx_{\rv{x} \sim \DShap}[f(\rv{x}) \neq f'(\rv{x})] &= \Prx_{\rv{x} \sim \DShap}[\sign(\ell(\rv{x})) \neq \sign(\ell'(\rv{x}))] \\
                       &\leq \Prx_{\rv{x} \sim \DShap}[|\ell(\rv{x})| < |\ell(\rv{x}) - \ell'(\rv{x})|] \\
                       &\leq \Prx_{\rv{x} \sim \DShap}[|\ell(\rv{x})| < {\textstyle \sum_{i=k}^n |w_i|}]  \\
                                         &\leq \Prx_{\rv{x} \sim \DShap}[|\ell(\rv{x})| < |w_{k/2}|] \\
                                         &\leq O((\log n)^{-1} \cdot \eps^2) \ , \\
\end{align*}
where the penultimate inequality follows by Equation~\eqref{eq:wk2-vs-w1wt} and the final inequality follows by applying \Cref{thm:shapley-anti-concentration}, with its parameters set to $r := |w_{k/2}|$, $k := k/2$, $\zeta := \zeta/6$, and $\eta := \eta$, since we chose $k \geq \eps^{-(6 + \zeta)}$.
Combining this with
%
%
%
%
Corollary~\ref{cor:cor-ub-shapley-by-l1},
\begin{align*}
\dShapley(f, f') &\leq O\Big(\sqrt{\log n \cdot \Prx_{\rv{x} \sim \DShap}[f(\rv{x}) \neq f'(\rv{x})]} + \frac{1}{\sqrt{n}}\Big) \\
                 &\leq O(\eps + 1/\sqrt{n}) \\
                 &= O(\eps) \ .
\end{align*}
We have shown that $\dShapley(f, f') \leq O(\eps)$ for some LTF junta $f'$ on $k - 1$ indices.
Call these indices $H$.
It follows that, for every set $H' \subseteq [n]$ of $k - 1$ indices with $H \cap S \subseteq H'$, there exists an LTF junta $f'$ on $H'$ satisfying $\dPS{S} \leq O(\eps)$.
It remains to show how to compute such a function $f'$, which we do by enumeration.

We can easily compute $H \cap S$ from $\card{H \cap S}$ since by \Cref{lem:monotonicity-shapley} the Shapley indices are monotone in the weights of $f$, i.e., $w_i \leq w_j$ implies that $\fc(i) \leq \fc(j)$.
So, our algorithm starts by guessing $\card{H \cap S}$, the number of input indices appearing in $H$. It then sets $H'$ to be the union of the $\card{H \cap S}$ indices $i \in S$ with largest values of $\fc(i)$ and $(k - 1) - \card{H \cap S}$ arbitrary indices from $[n] \setminus S$.

%
Our algorithm then enumerates a weights-based representation of each candidate LTF junta $f'$ on $H'$. Finally, it computes the (exact) Shapley values of each such $f'$, and computes $\dPS{S}(f, f')$. It outputs a weights-based representation of the first such $f'$ that satisfies $\dPS{S}(f, f') \leq O(\eps)$.

%
%
%
%
Therefore, because the algorithm guesses $\card{S} + 1$ values for $\card{H \cap S}$, because there are at most $2^{(k-1)k}$ different LTFs on $k - 1$ variables, and because the (exact) Shapley indices of each of these LTFs can be computed in $\red{k}^{O(k)}$ time, the algorithm runs in $(\card{S} + 1) \cdot 2^{O(k^2)} \cdot 2^{O(k)} = \red{n^{O(\log n/\eps^{12+2\zeta})}}$ time, and the theorem is proved.
\end{proof}

%

